Designing Virtual Reality Games for Grief: A Workshop Approach with Mental Health Professionals

Although serious games have been increasingly used for mental health applications, few explicitly address coping with grief as a core mechanic and narrative experience for patients. Existing grief-related digital games often focus on clinical training for medical professionals rather than immersive storytelling and agency in emotional processing for the patient. In response, we designed Road to Acceptance, a VR game that presents grief through first-person narrative and gameplay. As the next phase of evaluation, we propose a workshop-based study with 12 licensed mental health professionals to assess the therapeutic impacts of the game and the alignment with best practices in grief education and interventions. This will inform iterative game design and patient evaluation methods, ensuring that the experience is clinically appropriate. Potential findings can contribute to the design principles of grief-related virtual reality experiences, bridging the gap between interactive media, mental health interventions, and immersive storytelling.

==> related-works.tex <==
\section{Related Works}

\subsection{Grief and Digital Interventions}

Digital interventions have increasingly been explored for mental health applications, including grief processing. Prior research by Rolbiecki et al. \cite{rolbiecki2021digital} has investigated digital storytelling as a supportive tool for individuals who have experienced adverse life events, allowing them to process their emotions through narratives. For instance, storytelling has been used to help bereaved families make sense of their loss and develop new traditions and rituals, potentially reducing distress and improving their ability to support one another \cite{rolbiecki2017digital}. Based on both Rolbiecki et al.'s studies, benefits of digital storytelling for individuals processing adverse life events, such as the death of a family member, include an improved sense of self, enhanced self-efficacy, and improved quality of life. However, many of these interventions focus on passive engagement rather than interactive agency, leaving a gap in research on the role of gamified experiences in grief support.

\subsection{VR for Mental Health \& Grief Interventions}

Virtual Reality (VR) has been widely explored for mental health interventions, demonstrating efficacy in exposure therapy, stress reduction, and PTSD treatment. The immersive nature of VR can induce positive and pleasurable experiences, foster engagement and self-realization, and support and enhance interpersonal relationships, thereby promoting personal well-being \cite{pira2023use}. Some studies have investigated the use of VR in grief therapy, such as simulated conversations with deceased loved ones and guided grief exposure exercises. For example, VR interventions have been used to provide safe and immersive environments for individuals to learn coping strategies and manage conditions like anxiety and depression, which are often associated with grief \cite{jingili2023systematic}. However, concerns about ethical design, emotional safety, and long-term therapeutic effectiveness remain underexplored. This study builds upon these findings by integrating VR mechanics with evidence-based grief counseling principles to assess their impact on mental health professionals’ practices.

\subsection{Exploring Grief in Games}

Serious games have been increasingly utilized to explore complex emotions, including grief, loss, and trauma. Games such as \textit{Closer the Distance}\footnote{\url{https://store.steampowered.com/app/1991300/Closer_the_Distance/}} incorporate grief as a central narrative theme, providing players with opportunities for reflection and emotional catharsis. In VR, projects have experimented with embodied interactions to facilitate emotional processing through immersive storytelling. For example, VR interventions have been used to promote relaxation and reduce stress for adults with mental health conditions \cite{riches2023virtual}, which can be beneficial in processing grief. However, few VR experiences explicitly align with best practices in grief counseling or assess their therapeutic applicability through empirical studies. The present work addresses this gap by proposing an evaluation on how mental health professionals perceive and apply a grief-focused VR game in their practice.

==> system-description.tex <==
\section{System Description}

\textit{Road to Acceptance} has previously been introduced as an extended abstract in anonymous citation \cite{alvarenga2024road}. The mechanics of the game are based on the five-stage model of Kübler-Ross \cite{kubler2009five}. This paper explains the system in more detail and proposes a methodology for a future study to evaluate its effectiveness with mental health professionals.

The gameplay follows an episodic structure where players navigate key grief-related emotions through interactive storytelling. Each stage (denial, anger, bargaining, depression, acceptance) presents unique challenges that reinforce the emotional arc of grieving. Unlike traditional narrative-driven serious games, \textit{Road to Acceptance} leverages embodied VR interactions—such as symbolic actions (releasing objects, engaging in a dialogue with a NPC, revisiting memories)—to engage users in reflective and therapeutic activities.

\subsection{Mapping the Five Stages of Grief}

Embodied interactions + informed game level descriptions

Agency.

\subsection{Dialogue, Audio, and Narrative}

Containering emotions + therapeutic storytelling

To evaluate the effectiveness and therapeutic potential of the game, we propose a workshop-based study with psychosocial professionals.
